A unified framework for walking and running of bipedal robots

In this paper, we propose a novel framework capable of generating various walking and running gaits for bipedal robots. The main goal is to relax the fixed center of mass (CoM) height assumption of the linear inverted pendulum model (LIPM) and generate a wider range of walking and running motions, without a considerable increase in complexity. To do so, we use the concept of virtual constraints in the centroidal space which enables generating motions beyond walking while keeping the complexity at a minimum. By a proper choice of these virtual constraints, we show that we can generate different types of walking and running motions. More importantly, enforcing the virtual constraints through feedback renders the dynamics linear and enables us to design a feedback control mechanism which adapts the next step location and timing in face of disturbances, through a simple quadratic program (QP). To show the effectiveness of this framework, we showcase different walking and running simulations of the biped robot Bolt in the presence of both environmental uncertainties and external disturbances.

==> Body/further.tex <==
\section{Further Explanations}
The purpose of this section is to share useful equations and analysis with collaborators. To be removed in the original paper.
\subsection{Useful Equations}
Calculating the average speed yields:
\begin{align}\label{vrptov}
	x_{vrp,0} - x_0 = \frac{T v_x}{2 + \mathcal{R}\omega \frac{\tau_s+1}{\tau_s-1}},
\end{align}
holding similarly in the $y$-direction.
Using~\eqref{vrptov}, we can remove the initial VRP from the CoM trajectory during stance and express it based on $\mathbf{v}$.
The CoM position an speed at the end of the stance phase are substantial values, derived as:
\begin{align}
x_{T_s} &= \frac{2 \tau_s T v_x}{(\tau_s+1)(2 + \mathcal{R}\omega \frac{\tau_s+1}{\tau_s-1})} + x_0,\nonumber\\
\dot{x}_{T_s} &= \frac{\omega T v_x}{2 + \mathcal{R}\omega \frac{\tau_s+1}{\tau_s-1}}.\nonumber
\end{align}
The $y$-direction is the same.


==> Body/todo.tex <==
% ***** Optimization Problem *****
\section{PROPOSED RUNNING OPTIMIZATION PROBLEM}
% Motivation
We propose a framework to optimize steps in a running motion separately.
The optimization is done over the next $\vrp$ location and step timing, which are then used in a whole-body controller to generate the running gate.
% Steps


\subsection{Nominal Values}\label{subsection:nominal}
Given the desired average velocity $v = \begin{bmatrix} v_x & v_y&  0 \end{bmatrix}^T$, a nominal step can be characterized by its' length, $L_{nom}$, width, $W_{nom}$, and timing, $T_{s, nom}$ and $T_{f, nom}$.
% min and max
The robot's physics and environment restrict each of these values within a range with lower and upper bounds denoted by \textit{min} and \textit{max} subscripts.

% T hvr
From~\eqref{bouncing}, 
\begin{eqnarray}
T_{hvr,min} = \sqrt{8 B_{min}/g} \quad , \quad
T_{hvr,max} = \sqrt{8 B_{max}/g},
%T_{hvr,min} &= \sqrt{8 B_{min}/g},\nonumber\\
%T_{hvr,nom} &= \sqrt{8 B_{nom}/g},\nonumber\\
%T_{hvr,max} &= \sqrt{8 B_{max}/g}.
\end{eqnarray}
and we set $T_{hvr,nom} = \sqrt{4 (B_{min} + B_{max}) /g}$ to obtain $B_{nom} = (B_{min} + B_{max})/2$.

% T
The lower and upper bounds on $T$ respecting other variables ranges is therefore,
\begin{align}
    T_{low} = \max \{ &\frac{L_{min}}{|v_x|} - T_{hvr,max}, \frac{W_{min}}{|v_y|} - T_{hvr,max}, \nonumber \\ &\frac{2B_{min}}{|v_z|} - T_{hvr,max}, 
    %\sqrt{\frac{8 B_{min}}{g}}, 
    T_{min} \}\\
    T_{high} = \min \{ &\frac{L_{max}}{|v_x|} - T_{hvr,min}, \frac{W_{max}}{|v_y|} - T_{hvr,min}, \nonumber \\ &\frac{2B_{max}}{|v_z|} - T_{hvr,min}, 
    %\sqrt{\frac{8 B_{max}}{g}}, 
    T_{max} \}.    
\end{align} 
The nominal step duration must lie within $[T_{low}, T_{high}]$, and we select the middle point, $T_{nom} = 0.5 (T_{low} + T_{high})$.
% L and W
After selecting $T_{nom}$, the nominal step length and width can be found immediately:
\begin{align}
    L_{nom} &= v_x (T_{nom}+T_{hvr,nom}), \nonumber \\ W_{nom} &= v_y (T_{nom}+T_{hvr,nom}).
\end{align}

% omega
By solving $H_{nom} = (H_{min} + H_{max})/2$ in~\eqref{eq:H} and using $T=T_{nom}$, $\omega_{nom}$ is determined as well. 
% Conclusion
Putting these steps together, specifying the desired speed, $v$, is sufficient for obtaining nominal values for all design variables.




% *****************
% ***** Modes *****
% *****************
\subsection{Modes of Motion}\label{sec:modes}
In the previous sections, gaits were segregated to walking and running depending on a flight phase's existence.
We extend this trend to categorize motion in four groups and call them \textit{modes of motion} based on the CoM's altitude pattern.
This distinction is particularly useful in recognizing the effect of velocity on motion. 
The first three modes, \textit{LIPM walking}, \textit{walking}, and \textit{sneaking}, do not include a flight phase, $T_f=0$, while the last one is \textit{running} and involves non-zero flight phases.
We argue that each mode is associated with a frequency range and transiting between different modes is done by changing $\omega$ in consecutive steps (note that $\omega$ is kept constant during a single step).
% TODO: we haven't discuss transition

We study the altitude derived per~\eqref{com_stance} to introduce different motion modes,
\begin{align}\label{z_walk}
    z_t = \frac{e^{\omega t} +\Gamma_s \, e^{-\omega t}}{1+\Gamma_s}(z_{0} - z_{vrp,0}) +z_{vrp,0} \quad , \quad 0\leq t\leq T_S.
\end{align}
% TODO: this is just repeating \eqref{com_stance} for convenience. Better to be merged with another paragraph, or ... Too short and not that informative.
In the above, $z_0$ is the CoM height at the beginning of each step and is determined by physical characteristics, and $z_{vrp,0}=z_{cop,0} + g/\omega^2$ is given by~\eqref{def:vrp}.

% ***** LIPM Walking *****
Walking is classically defined as a gait in which at least one leg is in contact with the ground at all times~\cite{walkingdef}.
A simplifying assumption is to maintain a constant CoM height which is the principal assumption of the well-known \textit{Linear Inverted Pendulum Model (LIPM)}.
Using the natural frequency, $\omega=\omega_0=\sqrt{g/(z_0-z_{cop})}$ in~\eqref{def:vrp} yields $z_{vrp,0} = z_0$ that boils down~\eqref{z_walk} to $z_t=z_0$.
The general dynamics per~\eqref{linear_dynamics} is reduced to LIPM in this case, and we call the corresponding motion \textit{LIPM walking}.

% ***** Walking *****
If $\omega <\omega_0$, it follows from~\eqref{def:vrp} that the CoM is initially located below the VRP, $z_0 < z_{vrp,0}$, rises from $t{=}0$ to $t{=}T_s/2$, and then falls until it reaches the initial height, $z_{T_s} = z_0$, forming a sequence of vaults centered at contact points.
The described gait is the most compatible one with the nature,
% TODO: ref
and we will proof it's stability privileges in~\ref{subsection:nominal_res}.

% ***** Sneaking *****
In addition to the well-studied LIPM walking and the general walking gait, we introduce another subdivision of walking that we refer to as \textit{sneaking}.
Repeating the same procedure for $\omega > \omega_0$ shows that $z_0 - z_{vrp,0} > 0$; so, the CoM goes down at first and then rises.
% describe
% The higher frequency of sneaking compared to other types of walking leads to a shorter stance duration, which requires greater step length and width to keep moving at the same velocity.
%So, sneaking is a type of motion with no flight periods, quick and long steps, and the CoM is at the lowest height at the middle of each step.
% benefit
This motion avails in climbing down an uneven surface (C.F.~\ref{sec:uneven}), along with serving as a median phase in walk-run switching. 
% TODO: walk-run switching not discussed.

% ***** Running *****
%\subsection{Running}
Any motion with a non-zero flight duration in which both feet are lifted up, is referred to as running.
% TOASK: add or not? 'One of the main differences between walking and running is the alternation sequence of the ground-touching leg.'   
The stance dynamics resembles a spring continuing to go down after landing each foot for $T_s/2$, getting the closest to the ground straightly above the contact point before being pushed up and away from the stance foot for the second half of the period. 
At the end of the stance phase, the foot is lifted up and the CoM goes through a ballistic trajectory.     
To identify the concordant frequency range, note that the flight duration per~\eqref{T_f} must be positive, or equivalently $\dcm_{z,0} - z_{vrp,0} > 0$, which is only plausible when $\omega>\omega_0$. 

% Froud 
Terrestrial locomotors decide between walking and running based on the motion velocity, simultaneously transiting from walking to running as the pace increases.
Biologist have investigated various structural and metabolic triggers to explain the speed threshold between walking and running; though, none could concretely justify the speed-up and down switching simultaneously.
A dimensionless measure in continuum mechanics referred to as \textit{Froude number (Fr)} is propitious in quantifying the transition speed~\cite{froud}.
Defined as $Fr \coloneqq (v_x^2 + v_y^2)/(g \, d)$, where $d$ denotes the CoM distance from the contact point, Froude number builds upon the absolute velocity to leg length ratio.
% TODO: d is not clear
While walking at any Froude number smaller than $1$ is mathematically plausible, observations suggest a switching point of $Fr=0.5$ for many biped species such as humans~\cite{Fr_human} and birds~\cite{Fr_birds}.       
We compute $Fr$ and use the threshold of $0.5$ to elect walking or running given a desired forward velocity in this paper. 
\begin{subequations}\label{R}%TODO
	\begin{align}[left ={\mathcal{R} = \empheqlbrace}]
    	& 0 \quad &\text{if} \; Fr<0.5 \nonumber\\
    	& 1 \quad &\text{if} \; Fr<0.5 \nonumber
	\end{align}
\end{subequations}
% TODO: why???
% TODO: still not sure how to use Fr


